Talking-to-Build: How LLM-Assisted Interface Shapes Player Performance and Experience in Minecraft

With large language models (LLMs) on the rise, in-game interactions are shifting from rigid commands to natural conversations. However, the impacts of LLMs on player performance and game experience remain underexplored. This work explores LLM's role as a co-builder during gameplay, examining its impact on task performance, usability, and player experience. Using Minecraft as a sandbox, we present an LLM-assisted interface that engages players through natural language, aiming to facilitate creativity and simplify complex gaming commands. We conducted a mixed-methods study with 30 participants, comparing LLM-assisted and command-based interfaces across simple and complex game tasks. Quantitative and qualitative analyses reveal that the LLM-assisted interface significantly improves player performance, engagement, and overall game experience. Additionally, task complexity has a notable effect on player performance and experience across both interfaces. Our findings highlight the potential of LLM-assisted interfaces to revolutionize virtual experiences, emphasizing the importance of balancing intuitiveness with predictability, transparency, and user agency in AI-driven, multimodal gaming environments.

==> tables/anova.tex <==
\begin{table}[!htbp]
\centering
% \scriptsize
\setlength{\tabcolsep}{8pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}llll@{}}
\toprule
 Condition & \textbf{Item}   & \textbf{Effect Size} & \textbf{P-value} & \\ \midrule

\multirow{7}{*}{Game Experience} 
& Four conditions  &  .131 &  .002 $**$ \\
& Command Simple vs LLM Simple & .141 &  .003 $**$ \\
& Command Complex vs LLM Complex & .051 &  .078  \\ 
& Command Simple vs Command Complex & -.012 &  .176 \\ 
& LLM Simple vs LLM Complex & -.097 & .003 $**$ \\
& Command vs LLM & .116 & .009 $**$ \\
& Simple vs Complex & -.073 & .005 $**$ \\

\hline

\multirow{7}{*}{Usability} 
& Four conditions & .085 &  .013  $*$ \\
& Command Simple vs LLM Simple & .106 & .013 $*$ \\
& Command Complex vs LLM Complex & .004 &   .601    \\ 
& Command Simple vs Command Complex & -.004 &  .547  \\ 
& LLM Simple vs LLM Complex & -.127 & .000 $**$ \\
& Command vs LLM & .051 & .082 \\
& Simple vs Complex & -.069 & .010 $*$ \\
\bottomrule
\end{tabular}
}
\caption{The results from ANOVA analysis across conditions.} 
\vspace{-5.0mm}
\label{tab:anova}
\end{table}


% F-value for ANOVA:
% The F-value os ANOVA is a tool to help you to determine that, Is the variance between the means of two samples significantly different or not. The ratio of the between the groups and within the groups. It also helps us to find out the p-Value. The P-value is the probability of getting the result at least at the point where the null hypothesis should be true.

==> tables/anova_p_and_effect.tex <==
\begin{table}[htb!]
\setlength{\tabcolsep}{10pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
\multirow{2}{*}{Task} & \multicolumn{2}{c}{\textbf{Game Experience}} & \multicolumn{2}{c}{\textbf{Usability}} \\ \cmidrule(l){2-5} 
                      & Command          & LLM              & Command       & LLM           \\ 
\midrule
Simple                &  XXX (YYY)      & XXX (YYY)      & XXX (YYY)   & XXX (YYY)   \\
Complex               & XXX (YYY)      & XXX (YYY)      & XXX (YYY)   & XXX (YYY)   \\
All                   & XXX (YYY)      & XXX (YYY)      & XXX (YYY)   & XXX (YYY)   \\ \bottomrule
\end{tabular}
}
\caption{
\jpei{ANOVA statistics of P Values (Effect Size) for Game Experience and Usability across task complexity (Simple vs. Complex) and interface types (Command-based vs. LLM-powered).}
}
\label{tab:statistics_transposed}
\end{table}


==> tables/case_study_czech.tex <==
% \begin{table}[htb!]
% \centering
% \begin{minipage}{0.95\textwidth}
%     \centering
%     \includegraphics[trim=10cm 10cm 0cm 15cm, clip, width=0.8\textwidth]{figures/czech.png}
%     \vspace{0.5em} % 图片和文字之间留一点空白
% \end{minipage}
% % \centering
% % \resizebox{\columnwidth}{!}{
% % \begin{tabular}{@{}p{0.9\linewidth}@{}}
% % \toprule
% % \includegraphics[trim=10cm 10cm 0cm 15cm, clip, width=0.6\textwidth]{figures/czech.png}
% % \\ \midrule
% % \begin{tabular}[c]{@{}l@{}}
% \begin{minipage}{0.95\textwidth}
%     \raggedright
% \textbf{User}: Pridej na budovu strechu z cihel a dvoje dvere.\\
% (Add a brick roof and two doors to the building.)\\
% % \end{tabular}\\ \midrule
% % \begin{tabular}[c]{@{}l@{}}
% \textbf{LLM}: \underline{\textit{Reflection}}: Add a roof made of bricks and two doors to the building in Minecraft 1.11.2\\ 
% \underline{\textit{Planning}}: Step 1: Roof with bricks;
% Step 2: Adding two doors\\ 
% \underline{\textit{Instructions}}:\\ 
% % // Step 1: Create the foundation of the flag. \\
% 1. Postav střechu z cihel:
% \begin{verbatim}
% /setblock ~1 ~3 \~ minecraft:brick\_block 0\\
% /setblock ~1 ~3 ~1 minecraft:brick\_block 0\\
% /setblock ~1 ~3 ~2 minecraft:brick\_block 0\\
% /setblock ~1 ~3 ~3 minecraft:brick\_block 0\\
% /setblock ~1 ~3 ~4 minecraft:brick\_block 0\\
% /setblock ~2 ~3 \~ minecraft:brick\_block 0\\
% /setblock ~2 ~3 ~1 minecraft:brick\_block 0\\
% /setblock ~2 ~3 ~2 minecraft:brick\_block 0\\
% /setblock ~2 ~3 ~3 minecraft:brick\_block 0\\
% /setblock ~3 ~3 ~ minecraft:brick\_block 0\\
% /setblock ~3 ~3 ~1 minecraft:brick\_block 0\\
% /setblock ~3 ~3 ~2 minecraft:brick\_block 0\\
% /setblock ~4 ~3 \~ minecraft:brick\_block 0\\
% /setblock ~4 ~3 ~1 minecraft:brick\_block 0\\
% /setblock ~5 ~3 \~ minecraft:brick\_block 0\\
% \end{verbatim}
% % /fill 0 64 2 64 0 stone\\ 
% % // Step 2: Arrange the colored blocks for the flag design.\\ 
% 2. Přidej dvě dveře:

    

% /setblock ~2 ~1 \~  minecraft:wooden\_door 0 replace\\
% /setblock ~4 ~1 \~  minecraft:wooden\_door 0 replace

% \underline{\textit{Self-check}}: Tyto příkazy umístí cihlovou střechu na budovu a přidají dvoje dveře. \\ Přizpůsob si přesné umístění střechy a dveří dle potřeby. (These commands will place a brick roof on the building and add two doors.\\ Adjust the exact placement of the roof and doors as needed.) \\

% \bottomrule
% \end{minipage}
% }
% \caption{An example of multilingual compatibility: A User has successfully created a Dutch flag by asking in Dutch.''}\label{fig:case_study_dutch_flag}
% \end{table}

\begin{table}[htb]
\centering

% --- 先插入图 ---
\includegraphics[trim=10cm 10cm 0cm 15cm, clip, width=0.8\linewidth]{figures/czech.png}

\vspace{0.5em} % 图片和文字之间留白

% --- 然后排文字 ---
\begin{tabular}{p{0.95\linewidth}} 
\toprule
\textbf{User}: Pridej na budovu strechu z cihel a dvoje dvere. (Add a brick roof and two doors to the building.) \\

\textbf{LLM}: \textit{Reflection}: Add a roof made of bricks and two doors to the building in Minecraft 1.11.2.\\
\textit{Planning}: Step 1: Roof with bricks; Step 2: Adding two doors.\\
\textit{Instructions}:\\
1. Postav střechu z cihel(Build a roof out of bricks):\\
\texttt{%

/setblock ~1 ~3 ~ minecraft:brick_block 0\\
/setblock ~1 ~3 ~1 minecraft:brick_block 0\\
/setblock ~1 ~3 ~2 minecraft:brick_block 0\\
/setblock ~1 ~3 ~3 minecraft:brick_block 0\\
/setblock ~1 ~3 ~4 minecraft:brick_block 0\\
/setblock ~2 ~3 ~ minecraft:brick_block 0\\
/setblock ~2 ~3 ~1 minecraft:brick_block 0\\
/setblock ~2 ~3 ~2 minecraft:brick_block 0\\
/setblock ~2 ~3 ~3 minecraft:brick_block 0\\
/setblock ~3 ~3 ~ minecraft:brick_block 0\\
/setblock ~3 ~3 ~1 minecraft:brick_block 0\\
/setblock ~3 ~3 ~2 minecraft:brick_block 0\\
/setblock ~4 ~3 ~ minecraft:brick_block 0\\
/setblock ~4 ~3 ~1 minecraft:brick_block 0\\
/setblock ~5 ~3 ~ minecraft:brick_block 0\\
}\\
2. Přidej dvě dveře(
Add two doors):\\
\texttt{%
/setblock ~2 ~1 ~ minecraft:wooden_door 0 replace\\
/setblock ~4 ~1 ~ minecraft:wooden_door 0 replace
}\\
\underline{\textit{Self-check}}: Tyto příkazy umístí cihlovou střechu na budovu a přidají dvoje dveře. \\ Přizpůsob si přesné umístění střechy a dveří dle potřeby. (These commands will place a brick roof on the building and add two doors.\\ Adjust the exact placement of the roof and doors as needed.) \\
\bottomrule
\end{tabular}

\caption{An example of multilingual compatibility: A user successfully modified a Minecraft building in Czech.}
\label{fig:case_study_czech}
\end{table}


==> tables/case_study_fuzzy.tex <==
\begin{table}[htb!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l@{}}
\toprule
\includegraphics[trim=10cm 10cm 0cm 15cm, clip, width=0.6\textwidth]{figures/hallucintion_bedroom.png}
\\ \midrule
\begin{tabular}[c]{@{}l@{}}
\textbf{User}: buld a bedroom
\\

\end{tabular}\\ \midrule
\begin{tabular}[c]{@{}l@{}}
\textbf{LLM}: \underline{\textit{Reflection}}: Keywords: Build, Bedroom\\ 
\underline{\textit{Planning}}: Step 1: Build foundation;  
Step 2: Build walls;  
Step 3: Roof;  
Step 4: Exterior details;  
Step 5: Interior room structure;  
Step 6: Doors and windows;  
Step 7: Interior furniture;  
Step 8: Lighting and decoration  \\ 
\underline{\textit{Instructions}}:\\ 
% // Step 1: Create the foundation of the flag. \\ 
Step 1: Foundation  
/fill 10 4 10 15 4 15 planks\\

Step 2: Walls  
/fill 10 5 10 15 8 15 stone\\

Step 3: Roof  
/setblock 10 9 10 wooden_slab
/setblock 15 9 10 wooden_slab
/setblock 10 9 15 wooden_slab
/setblock 15 9 15 wooden_slab\\

Step 4: Exterior details  
Add windows and a door here\\

Step 5: Interior room structure  
/fill 11 5 11 14 8 14 air\\

Step 6: Doors and windows  
/setblock 12 5 10 wooden_door
/setblock 13 5 10 glass_pane
/setblock 14 5 10 glass_pane\\

Step 7: Interior furniture  
/setblock 12 5 13 bed
/setblock 14 5 12 crafting_table
/setblock 14 5 14 bookshelf\\

Step 8: Lighting and decoration  
/setblock 11 7 11 torch
/setblock 13 7 11 torch
/setblock 15 7 11 torch
/setblock 11 7 14 torch
/setblock 15 7 14 torch
/fill 0 64 2 64 0 stone\\ 
% // Step 2: Arrange the colored blocks for the flag design.\\ 

\underline{\textit{Self-check}}:  All coordinates are within (0-100)\\
Only Minecraft 1.11.2 compatible blocks used \\
Structure includes doors, windows, interior furniture, lighting\\
Design is symmetrical and aesthetic\\
No place holder \textless{}x\textgreater \textless{}y\textgreater \textless{}z\textgreater. // Done! Your Dutch flag is ready!\end{tabular} \\ 
\bottomrule
\end{tabular}
}
\caption{An example of fuzzy typying}\label{fig:case_study_fuzzy}
\end{table}

==> tables/case_study_horse.tex <==
\begin{table}[htb!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l@{}}
\toprule
\includegraphics[trim=10cm 10cm 0cm 15cm, clip, width=0.6\textwidth]{figures/horse with an armor.png}
\\ \midrule
\begin{tabular}[c]{@{}l@{}}
\textbf{User}: give me a horse with armour
\\

\end{tabular}\\ \midrule
\begin{tabular}[c]{@{}l@{}}
\textbf{LLM}: \underline{\textit{Reflection}}: To give you a horse with armor in Minecraft 1.11.2, we will need to summon a horse with a specific armor type.\\ 
\underline{\textit{Planning}}: Step 1: Summon the horse; 
Step 2:  Add armor to the horse \\ 
\underline{\textit{Instructions}}:\\ 
% // Step 1: Create the foundation of the flag. \\ 
/summon minecraft:horse \~ \~ \~ {Tame:1}\\ 
% // Step 2: Arrange the colored blocks for the flag design.\\ 
/summon minecraft:horse \~ \~1 \~ {ArmorItem:{id:"minecraft:diamond_horse_armor",Count:1}}\\
\underline{\textit{Self-check}}: Add coordinates are within (0-100); Correct Minecraft 1.11.2 block IDs; \\ No place holder \textless{}x\textgreater \textless{}y\textgreater \textless{}z\textgreater. // Done! Your Dutch flag is ready! \\
This command will summon a horse with diamond armor above the previously summoned horse. You can replace "diamond_horse_armor" with "iron_horse_armor" or "gold_horse_armor" for different armor types.\\
Executing these commands will give you a tamed horse with diamond armor. Feel free to adjust the commands if you'd like a different armor type or if you have any other preferences!
\end{tabular} \\ 
\bottomrule
\end{tabular}
}
\caption{An example of multilingual compatibility: A User has successfully created a Dutch flag by asking in Dutch.}\label{fig:case_study_dutch_flag}
\end{table}

==> tables/demographics.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{10pt}
% \small
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Demographic} & \textbf{Categories} & \textbf{Numbers of Participants (\%)} \\ \midrule
Gender & Female & 16 (53.3\%)
\\ 
 & Male & 13 (43.3\%)
\\
 & non-binary & 1 (3.3\%) 
 % & Non-binary & %1 (0.7\%)
\\
\hline
Age & 18-25 & 7 (23.3\%)
\\
 & 26-35 & 22 (73.3\%)
\\
 & 36-45 & 1 (3.3\%)
\\
%  & 46-55 & 0 (7.0\%)
% \\
%  & 65+ & 0 (2.3\%)
% \\
\hline
Education & High school degree or equivalent & 8 (18.6\%)
\\
 & Bachelor’s degree & 15 (34.9\%)
\\
 & Master’s degree & 16 (37.2\%)
\\
 & Doctorate or higher & 4 (9.3\%)
\\
% \hline
% Professional Domain & Health and Medical Science & 7 (16.3\%)
% \\
%  & Science, Technology, Engineering, Mathematics (STEM) & 14 (32.6\%)
% \\
%  & Business, Economics, and Law & 6 (14.0\%)
% \\
%  & Communication, Arts, Culture and Entertainment & 5 (11.6\%)
% \\
%  & Education and Social Science & 8 (18.6\%)
% \\
%  & Government and Public Sector & 2 (4.7\%)
% \\
% & Other & 1 (2.3\%) \\
\bottomrule
\end{tabular}
}
\caption{Characteristics of participants in the study. \todo{(need the data from this study)}}
\vspace{-3mm}
\label{table:demographics}
\end{table}

==> tables/efefct_size.tex <==
\begin{table}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{10pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lll@{}}
\toprule
 Condition & \textbf{Item}   & \textbf{effect size}\\ \midrule

\multirow{8}{*}{Game Experience} 
& Command Simple vs LLM Simple  & 0.59 \\
& Command Complex vs LLM Complex  & -0.33  \\ 
& Command Simple vs Command Complex &   0.25\\ 
& LLM simple vs LLM complex &  0.60\\
& Command vs LLM &  -0.51\\
& Simple vs Complex &  0.55\\

\hline

\multirow{4}{*}{Usability}  
& Command Simple vs LLM Simple  &    -0.48 \\
& Command Complex vs LLM Complex  &    -0.097   \\ 
& Command Simple vs Command Complex &   0.11 \\ 
& LLM Simple vs LLM Complex &  0.77 \\
& Command vs LLM & -0.46\\
& Simple vs Complex &  0.53\\
\bottomrule
\end{tabular}
}
\caption{\todo{Effect size of the results comparing LLM vs command-based interfaces across task complexity.} 
% (**$p$<.01, *$p$<.05)
}
\vspace{-3mm}
\label{tab:statistics}
\end{table}

% F-value for ANOVA:
% The F-value os ANOVA is a tool to help you to determine that, Is the variance between the means of two samples significantly different or not. The ratio of the between the groups and within the groups. It also helps us to find out the p-Value. The P-value is the probability of getting the result at least at the point where the null hypothesis should be true.



==> tables/main_result_v1.tex <==
\begin{table}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{10pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lll@{}}
\toprule
 Condition & \textbf{Item}   & \textbf{Mean  (SD)} \\ \midrule

\multirow{8}{*}{Game Experience}  & Command  (Simple)  &   3.07 (0.56)    \\
& Command  (Complex)  &   2.93 (0.7)  \\
& LLM  (Simple)  &   3.52 (0.58)   \\ 
& LLM  (Complex) &  3.197 (0.42) \\ 
& Command & 3.00 (0.57)\\
& LLM & 3.36  (0.43)\\
& Simple & 3.30 (0.42)\\
& Complex & 3.06 (0.42) \\

\hline

\multirow{8}{*}{Usability}  & Command  (Simple)  &   2.58  (0.88)   \\
& Command  (Complex)  &   2.47  (1.02)  \\
& LLM  (Simple)  &   3.12  (0.68)   \\ 
& LLM  (Complex) &  2.58  (0.74) \\ 
& Command & 2.52  (0.79)\\
& LLM & 2.85  (0.62) \\
& Simple & 2.85  (0.82) \\
& Complex & 2.52  (0.88) \\
\bottomrule
\end{tabular}
}
\caption{Descriptive analysis of the results comparing LLM vs command-based interfaces across task complexity. \jpei{I do not understand it.}
%  (**$p$<.01, *$p$<.05)
}
\vspace{-3mm}
\label{tab:statistics}
\end{table}


==> tables/multi_aspect_analytical.tex <==

\begin{table}[!ht]
\centering
\scriptsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lp{4cm}p{4cm}}
\hline
\textbf{Aspect} & \textbf{Command} & \textbf{Conversation} \\ \hline
Interaction Style & Direct commands with fixed syntax. & Natural conversation with an LLM assistant. \\ 
% (e.g., \texttt{build pyramid 3 6 9 5 stone 3}) 
% (e.g., "I want a red brick house")
Error Handling & Syntax errors and incorrect arguments leading to failed commands. & LLM provides correct syntax for commands, reducing errors \\ 
Creativity/Diversity & User frequently tests commands with different parameters and materials. & User describes desire in natural language, and LLM translates them into commands. \\ 
% (e.g., \texttt{build castle, summon dragon})
Request Complexity & Commands are manually typed and structured with precise parameters & LLM breaks down requests into structured commands, providing multi-step instructions. \\ 
Types of Actions & Heavy use of building commands (pyramids, castles, gardens, houses) & More variety, including summoning entities, placing decorative elements, and adjusting the environment \\ 
Error Recover & User repeats similar commands after failures or syntax issues & LLM corrects errors by guiding the user on proper command usage \\ 
Goal Orientation & Task-oriented, focused on executing Minecraft commands & More exploratory and conversational, experimenting with LLM suggestions \\ \hline
\end{tabular}
}
\caption{Multi-aspect Comparison of Direct Command Input vs. LLM-based Conversational Interaction in Minecraft.}
\label{tab:comparison}
\end{table}

==> tables/observation_command_v1.tex <==

% \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{@{}llll@{}}
% \toprule
% No & Command & Description & Condition \\ 
% \midrule
% 1  &  place x y z block\_type data\_value (e.g, [place 0 1 0 glass 3]       &   place a block at x y z(coordinates) with material and color number    &   1   \\
% 2  &  summon x y z entity\_type(animal, human)       &  summon a (animal/person) at x y z     &  1    \\ 
% 3  &  daytime time\_value[e.g, daytime 19000]       &   set up the daytime to 19:00    &   1   \\
% 4  &   tree x y z sapling_type      &  plant a tree with specific sampling type     &    1  \\ 
% 5  &   build ladder x y z height      &  build ladders at x y z     &    1  \\ 
% 6  &    place torch x y z     &    place a torch at x y z   & 1     \\ 
% 7  &   weather weather_type(rain, thunder, clear)      &  set up the weather to (rain, thunder, clear)    &   1   \\ 
% 8 &    fill x1 y1 z1 x2 y2 z2 block\_type     &   fill with blocks     &    2  \\ 
% 9 &    build pond x y z length width depth     & build a pond at x y z      &    2  \\ 
% 10   &   build castle x y z length width height block\_type   &  build a castle at x y z     &   2   \\ 
% 11 &   build house x y z length width height block\_type   &  build a house at x y z     &    2  \\ 
% 12 &   build garden x y z length width   &  build a garden at x y z     &    2  \\ 
% 13 &  build pyramid x y z base_size height block\_type    &  build a pyramid at x y z     &    2  \\ 

% \bottomrule
% \end{tabular}
% \end{table}

% \usepackage{tabularx}

% % 表格内容
% \usepackage{adjustbox}


\begin{table*}[!ht]
\centering
\scriptsize
\centering
\setlength{\tabcolsep}{1.5pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{No.} & \textbf{Command} & \textbf{Description} & Condition \\
\midrule
1  & \textbf{place} x y z block\_type color\_number      &   place a block at a position (x, y, z) with a specific material and color number (e.g, [place 0 1 0 glass 3] ).   &   1   \\
2  &  \textbf{summon} x y z entity\_type       &  summon a specific animal or person at a position (x, y, z)     &  1    \\ 
3  &  \textbf{daytime} time\_value       &   set up the daytime    &   1   \\
4  &   \textbf{tree} x y z sapling\_type      &  plant a tree with specific sampling type     &    1  \\ 
5  &   \textbf{build} ladder x y z height      &  build ladders at x y z     &    1  \\ 
6  &    \textbf{place} torch x y z     &    place a torch at x y z   & 1     \\ 
7  &   \textbf{weather} weather\_type      &  set up the weather to a specific type (i.e., rain, thunder, or clear)    &   1   \\ \midrule
8 &    \textbf{fill} x1 y1 z1 x2 y2 z2 block\_type     &   fill with blocks     &    2  \\ 
9 &    \textbf{build} pond x y z length width depth     & build a pond at x y z      &    2  \\ 
10   &   \textbf{build} castle x y z length width height block\_type   &  build a castle at x y z     &   2   \\ 
11 &   \textbf{build} house x y z length width height block\_type   &  build a house at x y z     &    2  \\ 
12 &   \textbf{build} garden x y z length width   &  build a garden at x y z     &    2  \\ 
13 &  \textbf{build} pyramid x y z base\_size height block\_type    &  build a pyramid at x y z     &    2  \\ 
\bottomrule
\end{tabular}
}
\caption{Observation commands and their descriptions for simple and complex tasks.}
\end{table*}



==> tex_files/introduction.tex <==
\section{Introduction}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Talking-to-build.png}
    \caption{An illutration of how LLM-Assisted Interface Shapes Player Performance and Experience in Minecraft.}
    \label{fig:motivation}
\end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[trim=0 0 0 160, clip, width=\linewidth]{figures/system design.png}
%     \caption{system design.}
%     \label{fig:motivation}
% \end{figure}
% ⛔️ @Charlotte could you write a draft with the following structure? Then XSUN will revise and adapt based on your inputs

The integration of large language models (LLMs) with interactive gaming environments represents a transformative frontier in both artificial intelligence and game research. This convergence not only advances scientific inquiry, but also holds significant social and technological implications. LLMs, having matured into powerful tools capable of both online and offline contextual reasoning, enable the development of autonomous agents that can engage in natural dialogue, collaborative problem-solving, and adaptive interaction within complex virtual worlds.
By bridging human intention with machine creativity, these intelligent agents facilitate dynamic collaboration, procedural content generation, and context-aware narrative design. On a broader level, the fusion of LLMs and games contributes to the evolution of digital ecosystems that are more intelligent, socially responsive, and capable of increasing education, research exploration, and user engagement. As this integration progresses, it is poised to redefine the boundaries of human-computer interaction and foster new forms of collaborative intelligence in both scientific and sociological domains.

% background of the current research: background, states of the arts
Some research show that conversational agent is able to collaborate in Minecraft to accomplish simple building tasks.  
% challenges and motivations
However, developing a conversational agent capable of effectively collaborating within an existing environment or platform, such as Minecraft, remains a significant challenge. This process involves integrating large language models (LLMs), which raises key concerns regarding the accuracy and reliability of natural language understanding, as well as the risk of hallucinations — situations where the model generates plausible but incorrect or irrelevant outputs.\\Additionally, it is not only a technical challenge to ensure that the conversational agent can correctly interpret and execute user commands; it is also critical to understand how the presence and performance of such an agent influence the users’ in-game performance, task completion efficiency, and overall gaming experience. These challenges motivate us to explore the delicate balance between LLM accuracy, user trust, system usability, and game immersion, aiming to build conversational agents that are not only technically robust but also enhance the user experience in complex, dynamic virtual environments.
% research questions and hypotheses if we have
There are three research questions:

\begin{itemize}
    \item \textbf{\textit{RQ1: Can LLM-assisted interaction in Minecraft enhance users' overall game experience and usability level while influencing their capabilities to execute commands?}}
\end{itemize}
% \subsection{RQ1: Can language-based interaction in Minecraft enhance users' overall game experience and usability level while influence their capabilities to execute commands}
In research question 1, we aim to investigate whether the integration of LLM-assisted interaction within the Minecraft environment can positively impact users' overall gaming experience and perceived usability of the system. Furthermore, we seek to examine whether such interaction mechanisms affect users’ efficiency, accuracy, and confidence in executing in-game commands.
Traditional Minecraft gameplay requires players to use a combination of manual controls and command-line syntax, which can pose challenges for new or casual users and create barriers to more complex in-game operations. The introduction of LLM-assisted interfaces offers the potential to bridge this gap by allowing players to express their intentions in natural language, thus improve their game experience and operability.

\begin{itemize}
    \item \textbf{\textit{RQ2: Does task complexity influence the performance of LLM in Minecraft on overall game experience and usability level and capabilities to execute commands?}}
\end{itemize}
% \subsection{RQ2: Does task complexity influence the performance of LLM in Minecraft on overall game experience and usability level and capabilities to execute commands?}
In research question 2, we plan to investigate whether the complexity of tasks will have a significant impact on the performance of large language models (LLM) in Minecraft. Additionally, we will further explore whether this impact will indirectly or directly affect users' overall gaming experience, system availability, and their ability to execute instructions in the game.
The task complexity in Minecraft can be manifested in various aspects, such as the number of task steps, the types of objects that need to be operated on, the complexity of spatial planning, or the difficulty of the problems to be solved. Tasks with higher complexity not only impose higher requirements on the model in terms of language understanding, interpreting, planning, reasoning, memory, and action generation, but also affect the users' trust and reliance on the model's output, thereby influencing the user experience and usage efficiency.
Through this research question study, we aim to deeply understand the moderating effect of the variable of task complexity on the relationship between model performance and user experience. Thus, it will provide theoretical basis and experimental references for subsequent optimization of the interaction strategies, task decomposition capabilities and auxiliary mechanisms of large language models in open virtual environments.

\begin{itemize}
    \item \textbf{\textit{RQ3: Does the ability of LLM-assisted interaction to execute commands moderate overall game experience in Minecraft?}}
\end{itemize}
% \subsection{RQ3: Does the ability of NLP-based interaction to execute commands moderate the overall game experience in Minecraft}
Research Question 3 serves as the core link between Research Question 1 and Research Question 2, aiming to explore a general effect, namely whether the performance of interaction methods based on LLMs in terms of executing instructions significantly moderates the overall gaming experience of players in Minecraft. In other words, we hope to clarify whether, when LLM can understand and execute natural language instructions in a more efficient and accurate manner, it will further enhance players' satisfaction, immersion, and the usability evaluation of the system. 
Furthermore, this research also focuses on the possible non-linear relationship between the model's execution ability and user experience: If LLM performs poorly in task execution, will it lead to users' frustration or a decline in their trust? Conversely, when LLM can still complete instructions with high quality under complex tasks, will it significantly enhance players' confidence, stimulate their desire for exploration, and enhance the immersion in the game?
By answering this research question, our aim is to establish a theoretical framework regarding the relationship among "model execution ability - user perception - game experience", and to provide valuable research references for future design of more intelligent and adaptable natural language interaction systems in virtual sandbox environments.\\

% what we did in this work
In this project, we developed a system that enables intelligent collaboration within the Minecraft environment to assist users in accomplishing various tasks. Users can freely input natural language commands through the Minecraft interface, and the system will automatically interpret and translate these commands. By integrating with the Malmo platform, the system transforms natural language instructions into executable actions, allowing seamless task execution within the game world.
% most important and interesting takeaways/findings from the study

% contributions and implications of this work
Scientifically, it explores the application boundaries of large language models (LLM) in open-ended virtual environments, especially in highly complex and dynamically changing Minecraft scenarios, by integrating natural language understanding with agent action decision-making. This provides a new experimental paradigm for cross-modal agent interaction research. Secondly, the study examines the impact of task complexity on model performance and user experience, which helps deepen the understanding of the relationships among various elements in the "language understanding-task planning-human-computer collaboration" chain. Moreover, this research also offers theoretical support and practical cases for how to deeply integrate conversational AI with complex instruction execution platforms, and has a promoting effect on the development of the intersectional fields of natural language processing, reinforcement learning, and human-computer interaction.\\ Socially, this research is conducive to promoting the application of natural language interaction technology in more extensive scenarios. Through exploration in the open virtual world of Minecraft, the research outcomes can provide references for fields such as education, games, virtual training, and auxiliary tools, helping to lower the threshold for using complex systems and enabling non-professional users to operate easily through natural language. Moreover, with the continuous strengthening of the trend of integrating virtual spaces with real-world scenarios, this research also has reference significance for future directions such as intelligent assistants, virtual world modeling, and human-computer co-creation, promoting the development of AI services towards more inclusive, intelligent, and user-friendly directions.

\todo{We list our contributions:
- Contribution 1;
- Contribution 2;
}

==> tex_files/related_work.tex <==
\section{Related Work}
% \jpei{Discuss related work in multiple paragraphs, each paragraph is one sub topic.}
% ⛔️ @Charlotte could you write a draft of this part?
\subsection{Conversational Agents in Minecraft}
There is already a relatively large amount of research on making a conversational agent in Minecraft to explore the interaction and the LLMs' application in games. In 2024, Rao et al.\cite{rao2024collaborative} presented a preliminary study on using LLM-driven non-player characters in a collaborative setting within a 3D game by designing a minigame within Minecraft where players collaborate with 2 NPCs powered by GPT-4 to complete a quest. The research validates that most prominent ones being the NPCs and the players filling the gaps in each other's skills, the NPCs finding a contextual way to communicate code failures, and the LLM generating sub-goals to facilitate collaboration. Two researchers supposed a chat bot 'Mason' to collaborate with the player in Minecraft, Mason can suggest the next suitable task for current situation via the conversation with the player and observation of the player’s information. It can also generate and customize structures. \cite{frankllm} Nonetheless, Takuma Ichikawa and Ryuichiro Higashinaka presented their model in \cite{ichikawa2023modeling}, their model can handle both action and utterance generation in a unified model, and they have tested in Minecraft to validated that their model can generate better utterance and actions than baselines. However, in 2019 and 2020, Anjali Narayan-Chen et al. supposed an interactive agent that can communicate and execute simple building tasks in Minecraft aims to make the agent being collaborative in Minecraft. \cite{narayan2019collaborative}\cite{jayannavar2020learning} Guanzhi Wang et al. mentioned the first GPT-4 powered agent VOYAGER that is able to learn lifelong and explore in Minecraft, \cite{wang2023voyager}which autonomously explores, builds a reusable skill library via code-as-policy, and iteratively improves to cope more complex tasks through environment feedback and self-verification. It significantly outperforms prior LLM agents in exploration, task mastery, and generalization.
\subsection{Autonomous Exploration and Task Solving with LLMs in Minecraft}
Zhu et al. proposed a set of actions that enables LLM to generate actions to provide to the agent to execute.\cite{zhu2023ghost}Their framework is based on LLM to generate actions by preceiving the context, which presents LLM's memorization in Minecraft. Shunyu Liu et al. proposed a framework that relies on a fine-tuned LLaMA-3 model that empowere with long-term planning, dynamic-immediate planning, and autonomous exploration capabilities in Minecraft. \cite{liu2024odyssey}However, they mentioned that LLM has hallucination issues, which decreases the agent's performances in Minecraft, in future work, they will consider retrieval-augmented generation to improve the performance, and integrate visual understanding to enable the agent to explore more in Minecraft. Chalamalasetti Kranti et al. present that they measured the agent's building task performance in Minecraft by comparing different LLMs, including GPT-4, Llama-3-70b, Llama-3-8b, Llama-3-8b (fine-tuned), and BAP (fine-tuned). GPT-4 performs the best among all these 5 LLMs for the builder action
prediction task in Minecraft. \cite{kranti2024retrieval}Chalamalasetti Kranti et al. mentioned that predicting suitable action generation is challenging since the agent is required to understand the context. Yue Wu et al. demonstrate SmartPlay as a baseline framework for evaluating the abilities of large language models (LLMs) as intelligent agents in collaborative game environments\cite{wu2023smartplay}. In their work, they introduced SmartPlay, a rigorous benchmarking suite designed to assess various capabilities of LLMs as agents.  Hao Li et al. proposed an advanced learning system: Auto MC-Reward, which consists of Reward Designer, Reward Critic, and Trajectory Analyzer these 3 components. This system can help to improve agent's exploration efficiency in Minecraft.\cite{li2024auto} Shuo Huang et al. presented a LLM-based framework Word2Minecraft for generating complex playable game levels in Minecraft based on structured scenarios. Word2Minecraft enables to change such as such as protagonist goals, antagonist challenges, and environmental settings by transferring narrative elements into spatial constraints. They evaluated their framework, and the result shows that GPT-4-Turbo outperforms GPT-4o-Mini in most areas.\cite{huang2025word2minecraft}Shiying Hu et al. presents a model Text to Building in Minecraft (T2BM) to validate the capabilities of LLMs on generating 3D  buildings by involving refining prompts, decoding interlayer representation, and repairing. \cite{hu20243d}It mainly focuses on refining prompts and the results show that this model can generate correct buildings in Minecraft with complete construction and consistent blocks via appropriate prompts. Junyeong Park et al. investigate a framework-MrSteve that has episodic memory, which addresses the problem of the shortage of long-term memory for the agent exploring Minecraft. The result shows that this framework did improve task solving and exploration efficiency in Minecraft.\cite{parkmrsteve}

% \subsection{Comparison to Existing Work}
Compared to prior research, our system emphasizes a broader linguistic flexibility and input tolerance, enabling users to engage naturally even with minor language errors or non-English inputs. While existing studies largely focus on goal completion and action generation, our findings highlight the importance of maintaining user trust and satisfaction by handling imperfect inputs gracefully and providing semantically reasonable responses.
